The PRISM Alignment Dataset: What Participatory, Representative and Individualised Human Feedback Reveals About the Subjective and Multicultural Alignment of Large Language Models

Human feedback is central to the alignment of Large Language Models (LLMs). However, open questions remain about methods (how), domains (where), people (who) and objectives (to what end) of feedback processes. To navigate these questions, we introduce PRISM, a dataset that maps the sociodemographics and stated preferences of 1,500 diverse participants from 75 countries, to their contextual preferences and fine-grained feedback in 8,011 live conversations with 21 LLMs. With PRISM, we contribute (i) wider geographic and demographic participation in feedback; (ii) census-representative samples for two countries (UK, US); and (iii) individualised ratings that link to detailed participant profiles, permitting personalisation and attribution of sample artefacts. We target subjective and multicultural perspectives on value-laden and controversial issues, where we expect interpersonal and cross-cultural disagreement. We use PRISM in three case studies to demonstrate the need for careful consideration of which humans provide what alignment data.

==> tabs/splash.tex <==
\begin{figure}
    \centering
    \includegraphics[width = 0.9\textwidth]{figs/Splash.png}
    \fontsize{8pt}{8pt}\selectfont
\setlength{\tabcolsep}{2pt}
\centering
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{llllllll} 
\multicolumn{2}{c}{{\cellcolor[rgb]{1,0.541,0.404}}\textbf{Human Participants}} &  &  &  &  & \multicolumn{2}{c}{{\cellcolor[rgb]{0.718,0.898,0.792}}\textbf{Large Language Models }} \\
\underline{Survey Participants} & 1,500 &  & \multicolumn{2}{c}{{\cellcolor[rgb]{1,0.761,0.298}}\textbf{Conversations }} &  & Total Providers & 6 \\ 
\multicolumn{1}{r}{\textit{With Conversations}} & 1,396 \tiny{(93.1\%)} & \textbf{$\Rightarrow$} & \underline{Total Conversations} & 8,011 & \textbf{$\Leftarrow$} & \underline{Total Models} & 21 \\
Birth Countries & 75 &  & \multicolumn{1}{r}{\textit{Unguided}} & 3,113 \tiny{(38.9\%)} &  & \multicolumn{1}{r}{\textit{Commercial API}} & 12 \tiny{(57.1\%)} \\
Reside Countries & 38 &  & \multicolumn{1}{r}{\textit{Controversy guided}} & 2,438 \tiny{(30.4\%)}&  & \multicolumn{1}{r}{\textit{Open Access}} & 9 \tiny{(42.9\%)} \\
Conversations / participant & 5.7\tiny{$\pm$1.0} &  & \multicolumn{1}{r}{\textit{Values guided}} & 2,460 \tiny{(30.7\%)} &  & Conversations / model & 1430.9\tiny{$\pm$171.1} \\ 
Models seen / participant & 13.9\tiny{$\pm$2.5} &  & Turns / conversation & 3.4\tiny{$\pm$1.6} &  & Unique raters / model & 924.3\tiny{$\pm$94.4} \\ 
\hhline{==~~~~==}
 &  &  & Total Interactions & 27,172 &  &  &  \\
 &  &  & Total Utterances & 68,371 &  &  &  \\
\hhline{~~~==~~~}
\end{tabular}
\caption{\small \textbf{The \ourdata alignment dataset at 
a glance.} In the first stage, 1,500 participants fill in the \textbf{Survey} with details of their background, familiarity with LLMs and stated preferences for fine-grained behaviours (\cref{sec:the_survey}). We present full demographic and geographic breakdowns in \cref{tab:full_demographics} and \cref{tab:full_geographics}). Almost all participants then progress to the second stage, where they converse with LLMs on topics of their choosing, rate the responses on a cardinal scale, and give fine-grained feedback (\cref{sec:the_convos}). There are 8,011 \textbf{Conversations} between participants (\img{figs/icons/circle-user-round.png}) and LLMs (\img{figs/icons/bot-message-square.png}), forming 27,172  \textbf{Interactions}, i.e., human messages met with a set of model responses. In the first turn, four model respond to the opening prompt (\img{figs/icons/circle-user-round.png}; \img{figs/icons/bot-message-square-green.png}, \img{figs/icons/bot-message-square-yellow.png}, \img{figs/icons/bot-message-square-red.png}, \img{figs/icons/bot-message-square-blue.png}). In subsequent turns, the conversation continues with two responses sampled from the highest-rated model at a non-deterministic temperature (\img{figs/icons/circle-user-round.png}; \img{figs/icons/bot-message-square-blue.png}). Overall, \ourdata contains 68,371 \textbf{Utterances}, i.e., 3-tuples of (human message, model response, score).%
}
\label{fig:splash}
\end{figure}

